VLS: Steering Pretrained Robot Policies via Vision-Language Models

Why do pretrained diffusion or flow-matching policies fail when the same task is performed near an obstacle, on a shifted support surface, or amid mild clutter? Such failures rarely reflect missing motor skills; instead, they expose a limitation of imitation learning under train-test shifts, where action generation is tightly coupled to training-specific spatial configurations and task specifications. Retraining or fine-tuning to address these failures is costly and conceptually misaligned, as the required behaviors already exist but cannot be selectively adapted at test time. We propose Vision-Language Steering (VLS), a training-free framework for inference-time adaptation of frozen generative robot policies. VLS treats adaptation as an inference-time control problem, steering the sampling process of a pretrained diffusion or flow-matching policy in response to out-of-distribution observation-language inputs without modifying policy parameters. By leveraging vision-language models to synthesize trajectory-differentiable reward functions, VLS guides denoising toward action trajectories that satisfy test-time spatial and task requirements. Across simulation and real-world evaluations, VLS consistently outperforms prior steering methods, achieving a 31% improvement on CALVIN and a 13% gain on LIBERO-PRO. Real-world deployment on a Franka robot further demonstrates robust inference-time adaptation under test-time spatial and semantic shifts. Project page: https://vision-language-steering.github.io/webpage/

==> rss_steerdp/sections/introduction-v1.tex <==
\section{Introduction-v1}
% what is the challenge?
A robot is trained to place a cup at the center of a table. During training, it succeeds reliably. \yiqing{Be more precise. Not 'during training', it should be 'when evaluated on the training distribution.' This clarifies that the issue is generalization, not learning capacity.} At test time, the task changes only slightly  \yiqing{Specify that it is the \textbf{test environment} or \textbf{spatial configuration} that changes, rather than just \textbf{the task} to highlight that the underlying motor skill remains applicable}: the cup must be placed closer to the edge of the table, aligned with another object, or positioned to avoid a newly introduced obstacle. Despite these minimal changes, the robot fails—hesitating, colliding, or placing the cup imprecisely. None of these variations requires a fundamentally new skill. \yiqing{We should elaborate on this point. We need to argue that these failures are not due to a lack of motor primitives, but rather a lack of context-aware goal specification. The policy has the 'how,' but the distribution shift confuses the 'where' or 'when.'} Yet together they reveal a persistent limitation of modern robot policies \yiqing{Let's tone this down slightly to avoid overclaiming. Frame it as a specific gap: high-capacity policies often struggle with precision and constraint satisfaction under OOD, which is the primary bottleneck for real-world deployment}: strong performance within the training distribution does not translate to reliable behavior under out-of-distribution conditions, which is essential for real-world deployment. 

% What is the gap? 
Recent advances in robot learning have produced powerful pretrained policies, particularly those trained with diffusion or flow-matching objectives, that demonstrate impressive in-distribution performance across diverse manipulation tasks. However, even these expressive generative policies often break down when test-time goals, environments, or task constraints deviate slightly from the training data. \yiqing{references here.} Addressing such failures through retraining or fine-tuning is costly, brittle, and impractical at scale. \yiqing{More references here. And beyond just being 'costly', let’s argue that attempting to solve goal mis-specification purely through increased data coverage is a fundamental mismatch. We should position steering as a more surgical and efficient alternative to brute-force scaling}.

% Our proposal
In this work, we propose Vision–Language Steering (VLS), a training-free framework for steering pretrained robot policies with a system that combine Large-Vision Models and Vision-Language Models as test time \textcolor{blue}{Add more details on the approach here, but keep it very high level}. Rather than modifying policy parameters, VLS treats steering as a control problem at inference time: a vision–language model (VLM) steers the action distribution of a frozen diffusion or flow-matching policy to bias behavior toward task-relevant outcomes \yiqing{We need a more technical term for \textbf{task-relevant outcomes} since this is the main contribution of the paper. How about 'task-aligned semantic constraints' or 'reward-informed distribution shifting'?}. Importantly, many out-of-distribution scenarios do not require learning new behaviors, but instead demand reweighting, recomposing, or constraining behaviors already present in the policy’s training distribution. \yiqing{One example here will be helpful}. Language provides a compact and expressive interface for specifying these control objectives without altering the underlying policy \yiqing{Rather than saying 'without altering the policy', emphasize that language provides a compositional interface that allows us to reweight and constrain learned behaviors at inference time, leveraging the innate modularity of the VLM}.

% Our insight
Our approach is inspired by recent progress in training-free control of large language models, where inference-time steering reshapes a pretrained model’s output distribution to elicit task-specific behavior \yiqing{Again, what is \textbf{task-specific behavior}? Be explicit: does this mean the execution of the same skill under environment variation, or satisfying additional geometric/semantic constraints?} without additional optimization. VLS draws an analogous perspective for robotics: instead of adapting policies through parameter updates, we control the action distribution of a generative policy at inference time. By leveraging VLMs to guide diffusion or flow-matching policies, VLS enables flexible and sample-efficient adaptation to out-of-distribution conditions while preserving the generality and robustness of the underlying pretrained policy. \yiqing{We already introduced the high-level idea in the previous paragraph, here let's go a little deeper into how we did it. One to two sentence is sufficient. For example: We utilize VLMs to perform semantic task decomposition and generate trajectory-differentiable reward functions that provide dense, context-aware guidance to the action-generation process.}.

% summary of contribution
\yiqing{I think the main contribution is two-fold. 1) environment-agnostic generalization: enabling frozen VLAs to adapt to changes in goals and scene geometry that require modified motion sequences (not just visual background changes). 2) training-free efficiency: achieving this adaptation without the computational overhead of fine-tuning. [TODO: i need shuo to verify if my understanding is correct]. If so, the related work and experiment section should explicitly benchmark against these two axes.}

% Evidence
To demonstrate the effectiveness of our approach \yiqing{Replace 'effectiveness' with more specific metrics. This will make the argument more grounded/stronger. I suggest focusing on 'generality' (handling new combinations of constraints) and 'inference efficiency' (the low overhead of our steering mechanism)}, we conduct extensive empirical evaluations across simulation and real-world benchmarks. On CALVIN, a steering-centric benchmark for long-horizon manipulation, VLS consistently outperforms prior methods, including ITPS and DynaGuide—the current state of the art—achieving an average improvement of x\% across all tasks, demonstrating more effective inference-time steering of pretrained policies. We further evaluate VLS on LIBERO-PRO, a challenging variant of the LIBERO benchmark that emphasizes compositional and out-of-distribution generalization, where VLS enables stronger performance on the same frozen pretrained policies when integrated with vision–language–action models. Finally, in real-world robotic experiments, we show that VLS improves a robot’s ability to follow user instructions and generalize to unseen task constraints, while supporting the composition of multiple language-specified objectives to solve complex, long-horizon manipulation tasks. 









% To address these issues, we propose a different approach: viewing inference-time guidance as combining trajectory-differentiable reward functions with a general pretrained policy. We combine the high-level semantic understanding of vision foundation models and vision-language models with the action generation capability of multi-task diffusion models, using differentiable rewards as an intermediate bridge to guide pretrained policies at test time in a training-free, zero-shot manner. Specifically, we use DINO + SAM to automatically extract key objects and keypoints from the scene, leverage VLMs to segment tasks into stages, and generate trajectory-differentiable reward functions for each stage. These functions take keypoints and partially denoised proposal trajectories as input, outputting scalar rewards to evaluate trajectory quality. During the diffusion policy's denoising process, we provide guidance at two levels:

% 1. At the gradient level, we use reward function gradients with respect to trajectories to modify the noise update direction, gradually pushing trajectories toward regions conforming to high-level objectives without changing model parameters.
% 2. At the distribution level, we propose a path distribution sampling method based on particle interaction systems, gradually "tilting" the diffusion model's transition kernel through potential functions, concentrating the sampling distribution in high-reward regions and enhancing exploration and diversity beyond gradient guidance.

% In summary, our method explores a middle path between ``retraining an end-to-end model" and ``explicitly solving constraint optimization problems." Compared to end-to-end training relying purely on conditioning, we "edit in real-time" the model's behavioral trajectories during inference through explicit, differentiable objectives. Compared to methods relying completely on VLM knowledge to solve constraint optimization problems through code, we leverage pretrained policies' intrinsic action generation capability to more naturally handle contact-dense, temporally complex manipulation tasks. Long-term, this ``steerable diffusion policy" paradigm provides a more scalable path for building general robotic systems that are both powerful and controllable, capable of continuously adapting to new tasks and constraints in open environments.
